Infinity: A Scalable Infrastructure for In-Network Applications

Network programmability is an area of research both defined by its potential and its current limitations. While programmable hardware enables customization of device operation, tailoring processing to finely tuned objectives, limited resources stifle much of the capability and scalability desired for future technologies. Current solutions to overcome these limitations simply shift the problem, temporarily offloading memory needs or processing to other systems while incurring both round-trip time and complexity costs. To overcome these unnecessary costs, we introduce Infinity, a resource disaggregation method to move processing to capable devices while continuing to forward as the original owner, limiting unnecessary buffering and round-trip processing. By forwarding both the processing need and associated data simultaneously we are able to scale operation with minimal overhead and delay, improving both capability and performance objectives for in-network processing.

==> introduction.tex <==
\section{Introduction}
%Why programmable HW is good
%Which are the current limitations regarding scalability and resource sharing
%Add some context and cite FlexNGIA - connect both worlds
Traditional networking equipment follows a fixed function design model (e.g., ASICs) typically optimized for a narrowly defined role, such as a datacenter, distribution, or core device. This design approach provides a refined high performance architecture with limited versatility outside pre-defined operational scopes. However, this limits the degree of potential innovation, requiring operators to implement solutions that align with often out-dated pre-coded characteristics of the network device. With the rise of edge and in-network computing, today's network falls short in providing adaptable and agile architectures due to archaic implementation limitations. 

To overcome these challenges, developments in network programmability enable dynamic solutions. On the hardware side, Open-Flow, P4, and Smart NICs enable operators to tailor network use to unique performance metrics needed for highly custom applications. On the software side, Network Function Virtualization (NFV) enables deployment of tailored network functions without the need for expensive physical devices such as firewalls, accelerators, or load balancers. Despite recent advancements to improve the agility, flexibility, resilience, and security of networking equipment through network function virtualization (NFV), this methodology is not a panacea. 

The challenge with NFVs is the disparate progression between the rapidly increasing pace of network transmission compared to the slower rate of development with host processing. Here, non-negligible amounts of processing are required by the network device to ensure proper forwarding, filtering, and processing for each traversing packet\cite{accelnet, accelTCP, tonic}, [ref Accelnet, Tonic, AccelTCP] .  With limits to Denard Scaling and the slowing of Moore's law, this disparity is a problem which will continue to limit the capabilities of networked systems\cite{mooreslaw,dennard}. Further, this disparity and increased load to process networking actions runs counter to the need to also execute business logic, increasing infrastructure costs. 

To address challenges in developing a fully-flexible internet architecture, we propose \textit{Infinity}, a programmable network architecture which abstracts networking hardware as virtual pools of packet processing resources for in-network processing.  Infinity ensures that Network Functions (NFs) can be deployed in pools of virtually infinite resource capacity by leveraging data plane dis-aggregation, scale-out techniques, and per-function tailored performance requirements. By enabling Infinity to dynamically trade performance and scalability, while ensuring efficient usage of the underlying data center infrastructure, enables development of network applications beyond the scope of single hardware systems.

With Infinity we enable the following contributions to improve current NFV deployments by leveraging programmable networking hardware:
\begin{itemize}
    \item Provide abstractions for building scalable and flexible NFs on top of programmable hardware, enabling high-performance processing while freeing computation resources on commodity hosts.
    \item Enable NFs to be deployed in virtual programmable hardware pools (VHPs), giving them the illusion of infinite computation resources and flexible composition of NFs and NF chains.
    \item Provides a mechanism to fully and efficiently utilize the network infrastructure within the data center.
\end{itemize}

%In . Recently, a new level of flexibility and dynamism has been enabled by the network function virtualization (NFV) paradigm, in which network functions (NFs) like load-balancers, firewalls, and network address translators (NAT) run virtualized on top of commodity hardware leveraging technologies like hardware virtualization [ref VMware, KVM], and containers [ref docker].  

%While the NFV model has indeed improved the agility, flexibility, resilience, and security on data centers and cloud networks [ref stateless, Cilium ...], it comes with some drawbacks. First, the networking speed is increasing at a much faster pace than host CPUs due to the end of Moore's law \cite{mooreslaw}, and the limits of Dennard Scaling \cite{dennard}. Second, recent works have shown that in order to process packets at speeds going from 10s to 100s of Gbps a non negligible amount of CPU resources on hosts is needed \cite{accelnet, accelTCP, tonic}, [ref Accelnet, Tonic, AccelTCP]. This is not ideal as this decreases the hosts capacity to execute business logic increasing the overall infrastructure costs.

%Programmable networking hardware (e.g., programmable switches and SmartNICs) has emerged as a response to the urgent need to provide new networking features in data centers and ensure fast adapting to costumer needs with high performance, and security while ensuring that host CPUs will have free processing capacity to run the most valuable workloads on the datacenters. However, programmable networking hardware also have constraints and limitations that need to be addressed in order to fully leverage their benefits. 

%One of the main constraints observed in the current programmable hardware implementations, be it programmable switches or SmartNICs \cite{tofino, bluefield, agilio} is the limited amount of fast memory available (i.e., SRAM) \cite{tea}. This effectively limits the number of concurrent flows that can be processed at high-speed on those devices \cite{silkroad}. The situation becomes even more dramatic, for stateful network function implementations where state maintained on SRAM sits on the critical path of the NF high-performance processing. We should also consider that those devices have a finite amount of processing resources available, which may limit the processing complexity and scale of NFs that can be deployed on those equipment. Finally, today we have a great variety programmable networking hardware (e.g., programmable swicthes, NPU, SoC, and FPGA based SmartNICs) each of them with different processing capabilities, functionalities and constraints. In this scenario, optimally utilizing and combining those equipment to produce optimal NF solutions is challenging \cite{flightplan}.

%Currently no system can provide both seamless scalability and resource disaggregation  ...

%To deal with those challenges and limitations in this vision paper we propose "Infinity", an architecture that aims to abstract a set of programmable networking hardware as virtual pools of packet processing resources that ensures that NFs can be deployed in pools of virtually infinity resource capacity. For doing so, we propose to leverage data plane disaggregation, scale-out techniques, and also the observation that different applications have different performance requirements, enabling "infinity" to trade-off performance and scalability while ensuring efficient usage of the underlying data center infrastructure (i.e., networking elements and hosts).

%Benefits/opportunities and challenges of our solution
%probably I should not name the system before we have an implementation of it...Naming just to make writing about it easier
%We expect this architecture to enable: 
    %better utilization of the overall infrastructure - How?
    %better scalability - How?
    %flexible composition of NFs leveraging diverse functionalities on the infrastructure (e.g., accelerators, different HW architectures) - How?
    %better infrastructure control due to virtual HW pool abstraction - How?




The remainder of this paper is organized as follows: In section \ref{sec:motivation} we frame the problem of fully flexible internet architectures by highlighting limitations with current programmable solutions.We then introduce our architectural solution, Infinity, and demonstrate how we address the limitations of current disaggregation and scalability solutions in section \ref{sec:solution} before providing examples of use cases in \ref{sec:use_cases}. In section \ref{sec:discussion} we propose future directions with Infinity to enable fully flexible architectures while also addressing limitations to our approach. Finally, in section \ref{sec:conclusion} we conclude the paper and discuss the next steps in the direction of realizing our vision.
